Exacerbating Algorithmic Bias through Fairness Attacks

Algorithmic fairness has attracted significant attention in recent years, with many quantitative measures suggested for characterizing the fairness of different machine learning algorithms. Despite this interest, the robustness of those fairness measures with respect to an intentional adversarial attack has not been properly addressed. Indeed, most adversarial machine learning has focused on the impact of malicious attacks on the accuracy of the system, without any regard to the system's fairness. We propose new types of data poisoning attacks where an adversary intentionally targets the fairness of a system. Specifically, we propose two families of attacks that target fairness measures. In the anchoring attack, we skew the decision boundary by placing poisoned points near specific target points to bias the outcome. In the influence attack on fairness, we aim to maximize the covariance between the sensitive attributes and the decision outcome and affect the fairness of the model. We conduct extensive experiments that indicate the effectiveness of our proposed attacks.

==> sections/Introduction-old.tex <==
\section{Introduction}
Machine learning models are shown to be susceptible to various types of adversarial attacks targeted to degrade the performance of machine learning models. Research in adversarial machine learning has mostly focused on targeting accuracy as a measure \cite{chakraborty2018adversarial,li2018security}. However, with the advancement of research in fair machine learning, attention has geared toward fairness measures and their importance. A broad area of research has arisen by proposing different fairness measures and definitions \cite{dwork2012fairness,hardt2016equality,NIPS2017_6995,10.1145/3194770.3194776,mehrabi2019survey}. It is important to have systems that are away from discriminatory behavior as these systems can be used in sensitive environments, such as courts to make bail decisions \cite{Dresseleaao5580}; thus, crucial to have measures and standards to ensure that artificial intelligence (AI) systems are fair. 

Similar to accuracy, fairness measures are important in machine learning research and can be targeted by adversaries for malicious intent. For instance, adversaries can attack models used in government and other sensitive agencies to make them appear unfair in order to depreciate their values and credibility. Some adversaries can even gain profit with such attacks off of biasing decisions for their benefit, in credit or loan applications for instance \cite{chen2019fairness}; therefore, thinking about ways these attacks could happen for designing more robust systems in the future is crucial. The goal is to have systems that are robust to fairness attacks; thus, it is important to consider attacks targeted toward fairness.

\textbf{Our contributions.} In this work, we propose data poisoning attacks that are able to target fairness. We propose two families of poisoning attacks. Those that target fairness only without having noticeable effects on accuracy to make them more subtle and undetectable, and those that affect both fairness and accuracy by injecting poisoned points during train time. Some adversaries may want to harm systems with regards to fairness and accuracy at the same time, while others might only consider fairness. In light of this, we introduce anchoring attack and influence attack on fairness techniques. In anchoring attack, we target fairness only without harming accuracy as much, while in influence attack on fairness, we target both accuracy and fairness measures by incorporating a loss function maximizing and attacking which would degrade fairness and accuracy.

Through experimentation on three different datasets with different fairness measures and definitions, we show the effectiveness of our attacks in achieving the desired goal of either affecting fairness only without significant harm on accuracy or accuracy and fairness at the same time. In addition, we incorporate different baseline models to evaluate different aspects of our attacks. We demonstrate that original data poisoning attacks designed to attack accuracy are not suitable for fairness attacks; thus, highlighting the importance of attacks designed for fairness specifically. We also compare our methods against concurrent work on adversarial attacks on fairness and show the effectiveness of our methods over them.




